Conditional Diffusion-Based Retrieval of Atmospheric CO2 from Earth Observing Spectroscopy

Satellite-based estimates of greenhouse gas (GHG) properties from observations of reflected solar spectra are integral for understanding and monitoring complex terrestrial systems and their impact on the carbon cycle due to their near global coverage. Known as retrieval, making GHG concentration estimations from these observations is a non-linear Bayesian inverse problem, which is operationally solved using a computationally expensive algorithm called Optimal Estimation (OE), providing a Gaussian approximation to a non-Gaussian posterior. This leads to issues in solver algorithm convergence, and to unrealistically confident uncertainty estimates for the retrieved quantities. Upcoming satellite missions will provide orders of magnitude more data than the current constellation of GHG observers. Development of fast and accurate retrieval algorithms with robust uncertainty quantification is critical. Doing so stands to provide substantial climate impact of moving towards the goal of near continuous real-time global monitoring of carbon sources and sinks which is essential for policy making. To achieve this goal, we propose a diffusion-based approach to flexibly retrieve a Gaussian or non-Gaussian posterior, for NASA's Orbiting Carbon Observatory-2 spectrometer, while providing a substantial computational speed-up over the current operational state-of-the-art.

==> acknowledgments.tex <==
\subsubsection*{Acknowledgments}
We would like to deeply thank the OCO-2/3 Science and Algorithm Teams.

We appreciate the TCCON teams, who measure and provide ground-based XCO$_{2}$ validation to the carbon cycle research community (\citep{de2014tccon}; \citep{te2022tccon}, \citep{liu2023tccon}; \citep{hase2022tccon}; \citep{kivi2014tccon}; \citep{weidmanntccon}; \citep{zhou2022tccon}; \citep{deutschertccon}; \citep{dubey2022tccon}; \citep{wunch2022tccon}; \citep{garcia2022tccon}; \citep{shiomi2022tccon}; \citep{strong2022tccon}; \citep{notholt2022tccon}; \citep{morino2022tccon_a}; \citep{morino2022tccon_b}; \citep{morino2022tccon_c}; \citep{sussmann2023tccon}; \citep{buschmann2022tccon}; \citep{sherlock2022tccon_a}; \citep{wennberg2022tccon_a}; \citep{wennberg2022tccon_b})

This work was funded by NASA grant: \textbf{80NSSC24K0763}.
